An Open Database of Lunar Regolith and Simulants Properties

Lunar regolith, the layer of unconsolidated material covering the Moon's surface, is central to the science and technology developed for the Moon, notably related to in-situ science investigations, resource utilization, surface infrastructure, and mobility systems. However, data on lunar soil properties remain fragmented across decades of mission reports, often in formats that are difficult to access or interpret. We present a newly compiled database of lunar regolith physical and geotechnical properties, including data collected by direct in-situ measurements from crewed missions, estimates inferred from surface interactions on the Moon and using remote sensing, as well as laboratory analyses of samples returned to Earth. The data collected include, among others, the angle of internal friction and cohesion (both Mohr-Coulomb model parameters), bulk density, and static bearing capacity, extracted from Luna and Apollo-era historical mission documentation all the way to contemporary Lunar programs. The dataset specifies the type and location of the tests from which each value was obtained. Our database also includes parameters for lunar regolith simulants, providing a direct link between mission data and laboratory studies. In addition to centralizing this information, we developed a user interface that facilitates data retrieval, filtering, and visualization. This interface enables users to generate customized plots for comparative analysis. Developed in an open-science perspective, it is designed to evolve in response to the community's needs. The database and its associated tools significantly enhance the accessibility and usability of lunar regolith and simulants data for scientific and engineering research.

==> Moon-Database-Manuscript_V2_arxiv/Moon-Database-Manuscript/colors_define.tex <==
\definecolor{brickred}{rgb}{0.8, 0.25, 0.33}
\definecolor{darkorange}{rgb}{1.0, 0.55, 0.0}
\definecolor{persiangreen}{rgb}{0.0, 0.65, 0.58}
\definecolor{persianindigo}{rgb}{0.2, 0.07, 0.48}
\definecolor{cadet}{rgb}{0.33, 0.41, 0.47}
\definecolor{turquoisegreen}{rgb}{0.63, 0.84, 0.71}
\definecolor{sandybrown}{rgb}{0.96, 0.64, 0.38}
\definecolor{blueblue}{rgb}{0.0, 0.2, 0.6}
\definecolor{ballblue}{rgb}{0.13, 0.67, 0.8}
\definecolor{greengreen}{rgb}{0.0, 0.5, 0.0}
\definecolor{razzmatazz}{rgb}{0.89, 0.15, 0.42}
\definecolor{ultramarine}{rgb}{0.07, 0.04, 0.56}
\definecolor{midnightgreen}{rgb}{0.0, 0.29, 0.33}
\definecolor{lavenderpurple}{rgb}{0.59, 0.48, 0.71}
\definecolor{bittersweet}{rgb}{1.0, 0.44, 0.37}
\definecolor{amaranth}{rgb}{0.9, 0.17, 0.31}
\definecolor{patriarch}{rgb}{0.5, 0.0, 0.5}
\definecolor{darkcandyapplered}{rgb}{0.64, 0.0, 0.0}
\definecolor{cadmiumgreen}{rgb}{0.0, 0.42, 0.24}
\definecolor{darkgreen}{rgb}{0.0, 0.2, 0.13}
\definecolor{deepcarrotorange}{rgb}{0.91, 0.41, 0.17}
\definecolor{deepcarmine}{rgb}{0.66, 0.13, 0.24}
\definecolor{maroon}{rgb}{0.69, 0.19, 0.38}
\definecolor{midnightblue}{rgb}{0.1, 0.1, 0.44}
\definecolor{lava}{rgb}{0.81, 0.06, 0.13}
\definecolor{ceruleanblue}{rgb}{0.16, 0.32, 0.75}
\definecolor{sacramentostategreen}{rgb}{0.0, 0.34, 0.25}
\definecolor{darkgreen}{rgb}{0.12, 0.3, 0.17}%
\definecolor{carmine}{rgb}{0.92, 0.3, 0.26}%

==> Moon-Database-Manuscript_V2_arxiv/Moon-Database-Manuscript/initialization.tex <==
\usepackage{colortbl}
\usepackage{wrapfig}

\usepackage{textcomp}

\usepackage{siunitx}[=v2]
\sisetup{
	detect-all,
	exponent-product = \cdot, 	% change exponent sign
}
\DeclareSIUnit\fps{fps}

\usepackage{csquotes}

%\usepackage{enumerate}
%\usepackage{enumitem}

\usepackage{nicefrac}

\renewcommand{\vec}[1]{\bm{#1}}
\let\vec\mathbf

\newcommand\TODO[1]{%
  {\fboxsep=.3ex\colorbox{brickred}{\textcolor{white}{\textsc{TODO}}}
  \textcolor{brickred}{#1}}%
}

\newcommand\red[1]{%
  \textcolor{black}{#1}%
}

\newcommand*\mean[1]{\bar{#1}}

\usepackage[
	nonumberlist, 
	acronym, 
	%section,
	nomain,
	nopostdot,
]{glossaries}

\newacronym{isru}{ISRU}{\textit{in-situ} resource utilisation}
\newacronym{gtb}{GTB}{GraviTower Bremen Pro} 
\newacronym{zarm}{ZARM}{Center of Applied Space Technology and Microgravity}
\newacronym{1g}{$1g$}{Earth gravity}
\newacronym{mug}{$\mu g$}{microgravity}
\newacronym{dem}{DEM}{discrete element methods}
\newacronym{iss}{ISS}{international space station}
\newacronym{afm}{AFM}{atomic force microscopy}
\newacronym{vdw}{vdW}{van der Waals}
\newacronym{lro}{LRO}{Lunar Reconnaissance Orbiter}
